Electronic structure of boron and aluminum $\delta$-doped layers in silicon

Recent work on atomic-precision dopant incorporation technologies has led to the creation of both boron and aluminum $\delta$-doped layers in silicon with densities above the solid solubility limit. We use density functional theory to predict the band structure and effective mass values of such $\delta$ layers, first modeling them as ordered supercells. Structural relaxation is found to have a significant impact on the impurity band energies and effective masses of the boron layers, but not the aluminum layers. However, disorder in the $\delta$ layers is found to lead to significant flattening of the bands in both cases. We calculate the local density of states and doping potential for these $\delta$-doped layers, demonstrating that their influence is highly localized with spatial extents at most 4 nm. We conclude that acceptor $\delta$-doped layers exhibit different electronic structure features dependent on both the dopant atom and spatial ordering. This suggests prospects for controlling the electronic properties of these layers if the local details of the incorporation chemistry can be fine tuned.

==> Electronic structure of delta layers/appendices.tex <==
% Supplementary information starts here
\clearpage
\widetext
\appendix

\section{Concentration Effects within DFT}
\label{app:conc-effects}
\begin{figure}
    \includegraphics[width=0.5\columnwidth]{fig-not-delta-layer.pdf}
    \caption{ 
    The band structure of a system with the same supercell as used throughout the work and the same concentration of dopants, but the dopants are scattered through the system instead of fixed in a $\delta$-doped layer.
    }
    \label{fig:not-delta}
\end{figure}

One factor complicating the use of DFT to predict the band structure of $\delta$-doped layers is disentangling the effect of the arrangement of dopants in a $\delta$ layer from the concentration effect of a finite number of dopants in a periodically repeated cell.
For the supercell illustrated in Fig.~\ref{fig:schematic}a and b, the concentration of dopants within the $\delta$-doped layer is 1/4 ML.
Within the entire cell, however, the concentration is \SI{7.64e19}{cm^{-3}}, a relatively high concentration for a typical semiconductor.
It might be expected that for this high level of concentration, we should see large induced valence bands, regardless of whether the boron atoms are forming a $\delta$-doped layer or not.
To test this effect, in Fig.~\ref{fig:not-delta}, we predict the band structure of the 2$\times$2 supercell used throughout the work with the same concentration of B dopants (Figs.~\ref{fig:schematic}a and b), but with the positions randomly determined, instead of forming a controlled $\delta$-doped layer.

The shape of the impurity bands is very similar to the predicted shape of a boron $\delta$-doped layer (see Fig.~\ref{fig:b-bands}a), with a doubling of the bands similar to what Carter \textit{et al.} report for two interacting phosphorus $\delta$-doped layers \cite{carter2013electronic} (indeed, given the setup of our structure, this could alternately be viewed as the band structure of two spatially separated $\delta$-doped layers with a 1/8 ML concentration of acceptors).
The magnitude of the impurity bands is somewhat reduced with a 1$\Gamma$ energy of 158 meV, compared to a 1$\Gamma$ energy of 248 meV in the $\delta$-doped structure.
This demonstrates that while a significant amount of the band structure can be attributed to the concentration effect of using a limited supercell within DFT, the magnitude and clarity of the structure is still related to the arrangement of atoms into a $\delta$-doped layer.
We expect a similar effect would be seen for an analogously randomized Al structure. 
Our current technique for measuring the $\delta$-doped layer electronic structure matches that of the literature with phosphorus $\delta$-doped layers \cite{carter2009electronic,carter2011phosphorus,drumm2013ab1,drumm2013ab2}.
These theoretical techniques have largely been subsequentally confirmed by experimental characterization \cite{miwa2013direct,mazzola2014determining,mazzola2014disentangling,miwa2014valley,mazzola2018simultaneous,holt2020observation}.
We thus have some confidence that while the impact of $\delta$-doped layers and the concentration of dopants in a DFT supercell are unavoidably somewhat entangled, our work nevertheless provides a useful first-order approximation of the electronic structure of boron and aluminum $\delta$-doped layers.


\section{Line features }
\label{app:line_features}
\begin{figure}
    \includegraphics[width=\columnwidth]{line-bands_v2.pdf}
    \caption{ 
    (a) Top view of the placement of dopant atoms making a line feature within a 2$\times$4 cell. (b) Band structure of boron $\delta$-doped line feature. (c)  Band structure of aluminum $\delta$-doped line feature.
    }
    \label{fig:line-feature}
\end{figure}

Radue \textit{et al.} noted that using AlCl$_3$ as an APAM precursor leads to the formation of large ``line'' structures, where AlCl fragments migrate to form a linear superstructure on the silicon surface~\cite{radue2021alcl3}.
We accordingly examine the band structure of $\delta$-doped layers with a linear structure of dopant atoms for both boron and aluminum, as shown in Fig.~\ref{fig:line-feature}.
While these line structures have not been observed in boron $\delta$-doped layers, they nonetheless provide a useful comparison to the observed aluminum structures.

The band structure of the boron line structure, shown in Fig.~\ref{fig:line-feature}a, combines the features of the relaxed ordered and disordered band structures shown earlier.
Similar to the fully relaxed, ordered structure, the 1$\Delta$ band is pulled to be the highest energy valence band, creating an inversion of the curvature around the $\Gamma$ point, and moving the VBM to 0.12 $\times$2$\pi$/a in the $X$ direction.
Similar to the disordered structure, however, the impurity bands exhibit no degeneracy with a separation of 23 meV between the 1$\Delta$ and 1$\Gamma$ band and 17 meV between the 1$\Gamma$ and 2$\Gamma$ band.
While the 1$\Delta$ band is highly flat with an effective mass of --1.64, the 1$\Gamma$ and 2$\Gamma$ bands are curved with effective masses of 0.51 and 0.61, respectively.
The exact values of the bands and effective masses are displayed in Table ~\ref{tab:b-line-energy-eff-mass}.
Overall, our results highlight that the exact band structure of boron $\delta$ layers is highly dependent on the exact placement of boron atoms.

In aluminum line structures, however, the top impurity band is moved dramatically up, as shown in Fig.~\ref{fig:line-feature}b. 
The 1$\Gamma$ band is moved to 468 meV above the bulk VBM, with a separation of 272 meV between it and the next 2$\Gamma$ band. 
%\quinn{TBD: Plausible explanation or better structure, does seem to be dependent on relaxed structure, I don't get high band for pure scf.}
Both the 1$\Gamma$ and 3$\Gamma$ bands are fairly flat, with effective masses greater than unity.
The 2$\Gamma$ band is curved, however, with an effective mass of only 0.4. 
This indicates that the aluminum line feature, which is favored in experiments, has dramatic results on the accompanying electronic structure.
The exact values for the impurity band energies and effective masses can be found in Table ~\ref{tab:al-line-energy-eff-mass}.
It should again be noted that these band structures were calculated at the GGA level and future work using more accurate approximations such as hybrid functionals would be useful to accurately determine the exact shift of the impurity bands, particularly relative to the larger band gap. 
We should also note that due to the periodic nature of these calculations, the line feature of four aluminum atoms is repeated in every supercell, but does not form a continuous line. 
Radue \textit{et al.} found that these line structures were typically only three aluminum atoms long~\cite{radue2021alcl3}, so the proposed line structure of Fig.~\ref{fig:schematic}d used throughout this work will likely be somewhat close to the experimentally realized structure. 

While this line leads to an unusual band structure when using aluminum acceeptors, our finding of an elevated 1$\Gamma$ band remains consistent even when a variety of methodologies are used.
We have examined the same line feature using rotated supercells as well as supercells extended in the further in the slab direction, increasing the distance between periodic images and still found either the same elevated band or a band spanning the entire width of the band gap.
To investigate whether this was due to unusual ordering of the atomic positions, we additionally ran ab-initio molecular dynamics (AIMD) at a temperature of 25 C for 0.5 ps and then measured the band structure, producing the same elevated band.
Finally, we also used SCAN pseudopotentials~\cite{yao2017plane}, which have been shown to improve the band gap estimation, which similarly produced a 1$\Gamma$ band which spanned the entire band gap.
While it seems likely that real world devices with this line feature will have a band structure more closely resembling those seen throughout the main text of this work, the multiplicity of methods giving the same results indicate that some interesting physics is at work in this case and further work is warranted.



\begin{table}
\centering
\caption{The energy and effective mass of bands in a Boron $\delta$-doped layer structure forming a line feature. Energies are given in units of meV, and effective masses are given in m$_e$. }
\label{tab:b-line-energy-eff-mass}
\begin{tabular}{l c c}
\hline 
Band & Energy at $\Gamma$ & Effective mass at $\Gamma$  \\

\hline 
1$\Delta$ & 186  &  --1.64\\
1$\Gamma$ & 163 & 0.61 \\
2$\Gamma$ & 146 & 0.51 \\
E$_{\rm F}$ & 33 & \\
E$_{\rm CB}$ & 581 &  \\
\hline
\end{tabular}
\end{table}


\begin{table}
\centering
\caption{The energy and effective mass of bands in an Aluminum $\delta$-doped layer structure forming a line feature. Energies are given in units of meV, and effective masses are given in m$_e$. }
\label{tab:al-line-energy-eff-mass}
\begin{tabular}{l c c}
\hline 
Band & Energy at $\Gamma$ & Effective mass at $\Gamma$  \\

\hline 
1$\Gamma$ & 468  & 2.13 \\
2$\Gamma$ & 196 & 0.40 \\
3$\Gamma$ & 133 &  4.85 \\
E$_{\rm F}$ & 77 &  \\
E$_{\rm CB}$ & 620 &  \\
\hline
\end{tabular}
\end{table}


